MetaGraspNet: A Large-Scale Benchmark Dataset for Scene-Aware Ambidextrous Bin Picking via Physics-based Metaverse Synthesis

Autonomous bin picking poses significant challenges to vision-driven robotic systems given the complexity of the problem, ranging from various sensor modalities, to highly entangled object layouts, to diverse item properties and gripper types. Existing methods often address the problem from one perspective. Diverse items and complex bin scenes require diverse picking strategies together with advanced reasoning. As such, to build robust and effective machine-learning algorithms for solving this complex task requires significant amounts of comprehensive and high quality data. Collecting such data in real world would be too expensive and time prohibitive and therefore intractable from a scalability perspective. To tackle this big, diverse data problem, we take inspiration from the recent rise in the concept of metaverses, and introduce MetaGraspNet, a large-scale photo-realistic bin picking dataset constructed via physics-based metaverse synthesis. The proposed dataset contains 217k RGBD images across 82 different article types, with full annotations for object detection, amodal perception, keypoint detection, manipulation order and ambidextrous grasp labels for a parallel-jaw and vacuum gripper. We also provide a real dataset consisting of over 2.3k fully annotated high-quality RGBD images, divided into 5 levels of difficulties and an unseen object set to evaluate different object and layout properties. Finally, we conduct extensive experiments showing that our proposed vacuum seal model and synthetic dataset achieves state-of-the-art performance and generalizes to real world use-cases.

==> temp/Cover_Letter.tex <==
Prof. Jingshan Li
Editor-in-Chief
IEEE International Conference on Automation Science and Engineering (CASE) 2022

Dear Prof. Li,

we wish to submit our work entitled "MetaGraspNet: A Large-Scale Benchmark Dataset for Scene-Aware
Ambidextrous Bin Picking via Physics-based Metaverse Synthesis" for consideration as regular paper in IEEE International Conference on Automation Science and Engineering (CASE) 2022.

In our work we address the highly complex and fundamental problem of autonomous bin picking.  
%Despite decades of robotic research the task still poses high challenges on vision-systems and limits the applicability of today's commercial systems. 
Many previous work have provided excellent work for specific tasks, however bin picking is a multi-stage complex problem and solving the problem from one aspect will miss the details of the other. Therefore, to tackle this big-diverse data problem, we propose a comprehensive dataset based on metaverse synthesis. To the best of our knowledge, this is the first study to introduce a large-scale photo-realistic multi-modal data pipeline together with grasps labels for a vacuum and parallel-jaw gripper, as well as high-level scene understanding and manipulation order reasoning. Despite our experiments showing the positive effect of having high realistic training data from simulation, in real-world systems the vision models are confronted with new objects, sensor noise, different lightning or other environmental conditions. Therefore, we also provide a real world evaluation and novel object test set, recorded in a realistic environment setting and fully annotated for object and grasp point detection. All together these datasets enable vision-systems to take the next towards multi-gripper usage and cognitive understanding of bin scenes expanding the applicability of future's commercial picking systems.

We believe that our proposed work targeting logistics and industry 4.0 strongly fits the scope of CASE and aligns well with previously published work such as "SynPick: A Dataset for Dynamic Bin Picking Scene Understanding" (Periyasamy, Schwarz, Behnke 2021) in CASE'21 and will with its practicality appeal to its readership from academia and industry equally.

We presented an early concept for our dataset as oral-only presentation at Conference on Vision and Intelligent Systems (CVIS 2021) together with a short early preprint (https://arxiv.org/abs/2112.14663). Motivated by the positive feedback from colleagues and other researchers, we significantly expanded our early concept of MetaGraspNet by adding more items, ambidextrous grasp labels, amodal segmentation masks,and real world data and evaluated our methods by performing extensive robot experiments. We confirm that the submitted manuscript is original, has not been previously published and is not currently in press, under review, or being considered for publication by any other conference or journal.

All authors have read and approved the manuscript being submitted, and agree to its submittal to CASE 2022.

Please address all correspondence concerning this manuscript to me at maximilian.gilles@kit.edu.

Thank you very much for considering our manuscript for publication.

Sincerely,

Maximilian Gilles
Institute for Material Handling and Logistics
Karlsruhe Institute of Technology (KIT)
Karlsruhe, Germany




==> temp/TODO.tex <==

-> @UW send Max script to transfer labels to COCO format (Done)
-> @UW send max layout label for figure
-> @Emily provide Max with script for Layout label
-> @UW and @KIT shrink wiriting to 8 pages
-> @UW ask prof. Wong if cover letter is okay
-> @KIT upload data, finish code repo
-> @KIT create coco format labels for (instance segmentation and semantic segmentation) Info : I will leave occlusion and depth untouched and add it as numpy array in the dataset. Too much changes needed to convert custom amodal segmentation mask in coco. Depth Numpy is needed anyway.



